Sub-millisecond Video Synchronization of Multiple Android Smartphones

This paper addresses the problem of building an affordable easy-to-setup synchronized multi-view camera system, which is in demand for many Computer Vision and Robotics applications in high-dynamic environments. In our work, we propose a solution for this problem -- a publicly-available Android application for synchronized video recording on multiple smartphones with sub-millisecond accuracy. We present a generalized mathematical model of timestamping for Android smartphones and prove its applicability on 47 different physical devices. Also, we estimate the time drift parameter for those smartphones, which is less than 1.2 msec per minute for most of the considered devices, that makes smartphones' camera system a worthy analog for professional multi-view systems. Finally, we demonstrate Android-app performance on the camera system built from Android smartphones quantitatively on setup with lights and qualitatively -- on panorama stitching task.

==> IEEE Sensors'21 smartphone sync(2)/src/01_intro.tex <==
\section{Introduction}
% - What is the problem?

Perception systems that employ synchronized stereo or multi-view camera networks give more opportunities than monocular systems in a wide variety of tasks: depth estimation~\cite{zhang2020du}, 3D reconstruction and rendering~\cite{bortolon2021multi, mildenhall2020nerf}, human pose estimation~\cite{qiu2019cross, dong2019fast, remelli2020lightweight}, especially in high-dynamic scenes. However, to build such a system, additional specialized equipment and expertise are required as well as special tools to provide their synchronization. Those requirements create an abyss between developed algorithms and end-user. 

% - Why is it important?

The active usage of smartphones and the constant growth of their capabilities in terms of sensors quality, camera, Inertial Measurement Unit (IMU), etc. and computational performance make them an affordable tool for usage in such technological pipelines, as it has been incessantly showcased during the last decade in AR/VR applications, robotics~\cite{mueller2021openbot}, and medicine~\cite{kornilova2021deep}. %;)

% - Why is it hard?


% In such a way, the difference between frames capturing could achieve 15 msec, which is crucial for high-dynamic environments. Thus, besides clock synchronization, simultaneous triggering of frame capture from both devices is required.

%  using standard network-based (NTP, PTP) or data-based approaches~\cite{faizullin2021twist}

Besides time synchronization between devices, moments of camera shots should also be synchronized to achieve better data quality. In professional cameras, it is usually implemented by hardware triggering, unavailable from the smartphone API. To achieve frame-level sync on smartphones, instead of triggering, one can align camera streams from continuous streaming mode. Assuming that stream rate is equal among devices, phase shifts of those periodical signals should be aligned. Existing works propose continuously reloading the camera module until the phase shift will be aligned~\cite{latimer2014socialsync} or requesting frames with different exposure times, which shifts phase to target one in a more controllable and deterministic way~\cite{ansari2019wireless}. Although the purpose of those works is on aligning phase shifts during preview mode and extracting still images from preview, video recording is more advantageous because of hardware codec optimizations (H264, H265) and it provides more frequent and continuous observations.

% Also, Libsoftwaresync experiments are limited to Google Pixel smartphones, not giving answers on the applicability of this technology for other smartphone models. An additional obstacle for applying this approach is a not-investigated frame timestamping model that requires manual tuning of frame period parameters for every smartphone.

% - What do we do?
Our work presents a fully automated Android application for recording synchronized videos and images from multiple Android smartphones with sub-millisecond synchronization accuracy. It is based on the phase shift alignment algorithm from the previous work~\cite{ansari2019wireless} and extends it with analysis of phase shift during switching between preview and video mode. We also formulate a general mathematical model of frame timestamping on Android devices and define an optimization problem for calculating model parameters (period, phase shift). We propose an effective algorithm to estimate those parameters and evaluate the algorithm on 47 physical devices. Synchronization accuracy of implemented Android application is quantitatively evaluated on setup with lights and qualitatively~--- on panorama stitching of a dynamic scene. The app is publicly available\footnote{\url{https://github.com/MobileRoboticsSkoltech/RecSync-android}}.

\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.97\textwidth]{fig/samsung_combo_drift.pdf}
    \caption{{\em Top-Left:} Difference of consecutive timestamps for Samsung Galaxy S9+. {\em Bottom:Left:} Its histogram resembling a Gaussian. {\em Right:} Drift coefficients (\SI{}{\milli\second} per minute) for 47 different smartphones from Firebase database in logarithmic scale using different amount of samples for phase estimation.}
    \label{fig:drift}
    \vspace{-4mm}
\end{figure*}

% Our work presents a fully-automated Android application for recording synchronized videos from multiple Android smartphones with sub-millisecond synchronization accuracy, based on phase alignment algorithm from the previous work~\cite{ansari2019wireless}, extending it with analysis of phase shift during switching between preview and video mode. We also formulate an optimization problem for phase parameters calculation and provide an algorithm for their calculation. The proposed algorithm is verified on almost 50 different Android devices from the Firebase service. For video synchronization, for all devices, phase stability was analyzed during the switch between preview and video recording mode, demonstrating that on the majority of devices, mode switch doesn't affect phase stability that allows making a synchronized video recording. Video synchronization accuracy was quantitatively evaluated on setup with lights and qualitatively~--- on panorama stitching of video with the dynamic scene. App for multiple smartphone recording is publicly available~--- \ak{link}. \ak{To the best of our knowledge}

% The main contribution of our work is as follows:

% \begin{itemize}
%     \item mathematical model for frame timestamping and algorithm for phase parameters estimation;v
%     \item Android-app for synchronized video recording with sub-millisecond accuracy on identical smartphone models;
%     \item phase drift for almost 50 Android smartphones was calculated;
%     \item analysis of what smartphone combinations of different models could be used for low-drift synchronization.
% \end{itemize}


==> IEEE Sensors'21 smartphone sync(2)/src/02_related.tex <==
\section{Related work}

Camera synchronization of multiple smartphones deals with two main issues: clock synchronization in sensor networks and camera phase alignment. Approaches for clock synchronization could be divided into the following groups: (1) hardware synchronization using wires and special boards~\cite{tschopp2020versavis, liu2021matter}, usually not applicable to smartphones, (2) network-based approaches in which sensor nodes exchange timing messages via the network and aggregate statistics (NTP~\cite{rfc4330}, PTP~\cite{ptp2008}, RBS~\cite{rbs2006}), (3) data-based approaches based on aligning time of some event registered by data from all sensors~\cite{sandha2019exploiting}, for example, flashlights~\cite{vsmid2017rolling}, sound~\cite{ono2016self, sandha2019exploiting}, shake~\cite{faizullin2021twist}. Besides the topic of camera phase synchronization is well investigated in the professional equipment domain, the smartphone case is complicated by a variety of models and high-level API and was studied only in a couple of works. Among camera phase alignment approaches, SocialSync~\cite{latimer2014socialsync} and libsoftwaresync~\cite{ansari2019wireless} could be highlighted that employ different techniques for shifting camera phase.

%\subsection{Libsoftwaresync}

As the basis of our work, we use the libsoftwaresync approach of synchronized photo capturing with sub-milliseconds accuracy, which consists of two steps: (1) perform clock synchronization between smartphones using min-filtering NTP modification, (2) align camera phases of all devices to a common one using additional requests of frames with different exposure to shift the phase during preview mode.

% \gf{this paragraph can be reduced}
There are \textbf{two open questions} to which our research tries to give answers: (1) could this approach be extended to video recording (which is equivalent to phase stability after switch from preview to video mode) and (2) could this approach be scaled to the whole Android smartphone family and what is the amount of drift for common devices.

% There are \textbf{two open problems} to which our research tries to give answers: \gf{use positive sentences, or question} (1) this approach could not be scaled to video until camera module behavior after switching between preview and video mode will not be investigated, (2) this approach could not be scaled to whole Android smartphone family until timestamping process will not be investigated in different modes on a wide variety of smartphones.

% SocialSync uses camera module reloading that shifts phase until target phase is achieved.  

% \subsection{Libsoftwaresync}
% Libsoftwaresync proposes an effective way of aligning frame phases during preview mode by capturing frames with different exposure times. Thus continuing that process several times, the phase could be optimized to the target one.

% Libsoftwaresync app contains two steps: (1) perform clock synchronization between nodes using min-filtering NTP modification, (2) align camera phases of all devices to a common one using additional requests of frames with different exposure to shift the phase. The last step requires the frame period to be identical among devices in the system satisfied by using smartphones of the same model.


==> IEEE Sensors'21 smartphone sync(2)/src/04_android_phase.tex <==
% \section{System Overview}
% \gf{here include requirements, assumptions, maybe?}
% \ak{God of sections :)) we are less in space

% \subsection{Clock Sync}
% Clock sync between smartphones is well investigated and demonstrates sub-millisecond accuracy using either NTP modifications~\cite{ansari2019wireless} or gyroscope-based algorithm~\cite{faizullin2021twist}.

% \subsection{Setup}
% \label{sec:criteria}

\section{Camera phase analysis}
\label{sec:requirements}
In our work, we consider a system that contains multiple Android smartphones of the same model with Camera2API support and precise timestamping of frames that is guaranteed by properties of the camera metadata~\cite{cameradoc}. We assume the task of clock synchronization between smartphones to be solved as it was demonstrated in \cite{ansari2019wireless, faizullin2021twist} and focus on phase shift stability during switch to video recording.

% \gf{where do we say that time sync is solved? RW?}

\subsection{Problem formulation}

For each smartphone in multi-view camera setup, we solve the following problem independently. The instant of time $t_i$ is the {\em observed} moment when an image is captured, according to the camera timestamp. One can define a model of periodical timestamping, similarly as proposed in \cite{ansari2019wireless}:
\begin{equation}
    t_i = \tau_0 + N_i \cdot \tau + \eta_i, \label{eq_timestamping}
\end{equation}
where $\tau_0\in \mathbb{R}$ is the phase shift of the $i$th captured frame $i=1,\ldots,s$ and $\tau \in \mathbb{R}$ is the constant period between consecutive frames captured by the camera module. The integer $N_i \in \mathbb{N}$ is the frame index, which considers potential frame drop ($i\neq N_i$) and $\eta_i \sim p(\tau_0,\tau, N_i)$ is a random variable distributed according to some Probability Density Function (PDF). 

% \ak{move this to algorithm} One can define the finite difference of timestamps:
% \begin{equation}
%     \Delta t_i = t_i - t_{i - 1} = (N_i - N_{i - 1}) \tau + \eta_i - \eta_{i-1} = \Delta N_i \tau + \xi_{i},\label{eq_finit}
% \end{equation}
% where we {\em assume} that the new random variable $\xi_i$ to be Gaussian, as discussed in detail in Sec.~\ref{sec_noise}.

Consequently, the joint estimation problem for the phase shift $\tau_0$, the period $\tau$, and each of the integers in $\{N_i\}^{i=1, ...s}$ can be described as a constrained least-squared optimization model:
\begin{align}
    \min_{\tau_0, \tau, N_1,.., N_s} \sum_{i=1}^{s} (\tau_0 + N_i \cdot \tau - t_i)^2 \label{eq_problem_raw}\\
    \text{s.t.} \quad \tau\left(N_i - 0.5\right) \leq t_i \leq \tau\left(N_i + 0.5\right). \label{eq_constr}
\end{align}

The objective function represents the minimum square error between timestamp $t_i$ and timestamping model \eqref{eq_timestamping}. The constraint \eqref{eq_constr} depicts the timestamping bounds.
Due to the integer nature of $N_i$, this problem is classified as Mixed-Integer Problem (MIP) model. Off-the-shelf solvers, such as Gurobi or CPLEX, are the state-of-the-art tools for providing solutions to MIP problems. However, in practice, such solvers are not adequate for online decision-making \cite{bertsimas2019online} and not suited to be embedded into the mobile phone. 
%% DP: if length requires to cut, please cut the next paragraph. 
The interest in this type of problem has been materialized in developing initiatives for creating a new family of solvers for MIP models that require solving in short periods \cite{miosqp}. 


% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.99\columnwidth]{fig/samsung.pdf}
%     \caption{{\em Bottom-Left:} Difference of consecutive timestamps for Samsung Galaxy S9+. {\em Bottom-left:} Its histogram resembling a Gaussian.}
%     \label{fig:samsung}
% \end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\columnwidth]{fig/phase-noise.pdf}
    \caption{{\em Left:} Difference of consecutive timestamps for HTC 10. {\em Top-Right:} Its histogram showing different modes. {\em Bottom-Right:} Histogram of clustered sequences, now Gaussian.}
    \label{fig:htc}
%\vspace{-3mm}
\end{figure}

%This straightforward formulation of the problem requires solving a Mixed Integer Problem \gf{DAVID TODO}, which is computationally involved \gf{cite some sovlers?} and therefore not suited to be embedded into the mobile phone.

The optimization model \eqref{eq_problem_raw}--\eqref{eq_constr}  can be {\em exactly} reformulated into an unconstrained optimization problem. By manipulating the constraint inequalities in (\ref{eq_constr}), it is possible to obtain the exact equality for $N_i$,
\begin{equation}
    N_i(\tau) =  \floor*{\frac{t_i}{\tau} + 0.5},
    \label{eq_round}
\end{equation}
where the operator $\floor*{.}$ indicates the floor operator.
%By doing so, the original MIP problem \eqref{eq_problem_raw}--\eqref{eq_constr} becomes an ordinary least squares problem. In Sec.~\ref{sec_phase_alg} we will show further simplifications.

% \begin{equation}
%     \min_{\tau_0,\tau} \quad \sum_{i=1}^{s} \left(\tau_0 + N_i \cdot \tau - t_i\right)^2.
%     \label{eq_problem}
% \end{equation}

% \begin{equation}
%     \min_{\tau_0,\tau} \quad \sum_{i=1}^{s} \left(\tau_0 + N_i(\tau) \cdot \tau - t_i\right)^2.
%     \label{eq_problem}
% \end{equation}

% \ak{Next exact reformulation}

% \begin{align}
%     \min_{\tau_0,\tau} \quad \sum_{i=1}^{s} \left(\tau_0 + N_i(\tau, \tau_0) \cdot \tau - t_i\right)^2 \\ 
%     N_i(\tau, \tau_0) =  \floor*{\frac{t_i - \tau_0}{\tau} + 0.5} \\
%     0 \leq \tau_0 < \tau 
% \end{align}

% \ak{This LSQ formulation is complicated by complex model of $N_i(\tau, \tau_0)$, but in our case we could estimate it in the following way (knowing that minimum delta is usually around period and that clusters of timestamps are located far enough)}

% \begin{align}
%     \Delta t_i = t_{i + 1} - t_i, \quad
%     \tau_{init} = \min_{i \in [1, s-1]} \Delta t_i \\
%     N^{approx}_i = \floor*{\frac{t_i}{\tau_{init}}}
% \end{align}

% \ak{Then the problem becomes standard LSQ}

% \begin{align}
%     \min_{\tau_0,\tau} \quad \sum_{i=1}^{s} \left(\tau_0 + N^{approx}_i \cdot \tau - t_i\right)^2 
% \end{align}

\subsection{Approximated problem reformulation}\label{sec_phase_alg}

% Following the idea of clustering from timestamping properties, we propose the next algorithm that solves the described optimization problem. It consists of two steps: (i) initial phase estimation, (ii) phase refinement using cluster-based algorithm. Firstly, initial phase estimation is calculated as described in (\ref{eq:init-phase}). \gf{this is IEEE refernece to eqs} Then, the set of clusters $K=\{K_1,..,K_m\}$ is defined where the cluster contains $K_i$ a subset of $\Delta t_i$ that lie in the interval $((i-0.5)\tau_{init}, (i+0.5)\tau_{init})$ \gf{I would remove this and just explain the idea of breaking and solving N-LSQs}. Finally, the period of timestamps is calculated as a weighted sum of cluster means as described in Eq.~\ref{eq:period}, where $\overline{K_i}$ denotes mean of cluster $K_i$ samples and $|K_i|$~--- cardinality of cluster $K_i$. Finally, phase shift is calculated as described in Eq.~\ref{??}.

% \gf{some of the symbols not defined... this is out #1 candidate to remove.} \gf{tau est -- $\tilde{\tau}$ and $ = \mathbb{E}_{K}\{\tau_k\}$ where $\tau_k$ is the estimation to the subproblem as in (\ref{eq_problem})}
% \begin{align}
%     \label{eq:init-phase}
%     \Delta t_i = t_{i + 1} - t_i, \quad
%     \tau_{init} = \min_{i \in [1, s-1]} \Delta t_i \\
%     \label{eq:period}
%     \tau^{est} = \frac{1}{\sum_{i=1}^{m} |K_i|} \sum_{i=1}^m \frac{\overline{K_i}}{i} \cdot |K_i|
%     \label{eq:shift}
%     \tau_0^{est} = \frac{1}{s} \sum_{i=1}^s{(t_i - \floor*{\frac{t_i}{\tau^{est}}} \tau^{est})}
% \end{align}
The problem statement in \eqref{eq_problem_raw}--\eqref{eq_constr} could be approximated by estimating the $N_i$ and removing its dependency on $\tau$ by: 
\begin{align}
    N_i \approx \floor*{\frac{t_i}{\tau_{init}} + 0.5}, \quad \text{s.t.} \quad
    \tau_{init} = \min_{i} \Delta t_i.
\end{align}

One can further simplify the problem \eqref{eq_problem_raw} by considering finite differences between two consecutive image captures \eqref{eq_finit}:
\begin{equation}
    \Delta t_i = t_i - t_{i - 1} = (N_i - N_{i - 1}) \tau + \eta_i - \eta_{i-1} = \Delta N_i \tau + \xi_{i},\label{eq_finit}
\end{equation}
where we {\em assume} that the new random variable $\xi_i$ is distributed according to normal distribution $\xi_i \sim \mathcal{N}(0, \sigma(\Delta N_i, \tau))$, as discussed in Sec.~\ref{sec_noise}. In that case, the minimization problem could be formulated as in \eqref{eq:delta_min_problem} and could be decomposed into the sum of Least Square (LSQ) problems over the clusters associated with values of $\Delta N_i$. In that case, for every subproblem, the Gaussian assumption over the noise is satisfied therefore every subproblem could be solved using standard methods using the Gauss-Markov theorem. Finally, $\tau$ is calculated as a weighted sum of the subproblem's solutions. 

\begin{equation}
    \label{eq:delta_min_problem}
    \min_{\tau} \sum_{i=1}^{s} (\Delta N_i \tau - \Delta t_i)^2 = \min_{\tau} \sum_{k=1}^{\max N_i} \sum_{\Delta t_i \,\, \text{s.t.} \,\, k = N_i} (k \tau - \Delta t_i)^2
\end{equation}

% \mf{Overall, I would state clearly: we divide clusters to have T, 2T, 3T, etc inside every cluster cause it is natural idea due to clear difference between noise and loss}

\subsection{Noise Model}\label{sec_noise}

In this section, we justify the choice for a Gaussian distribution which resulted in the estimation problem in \eqref{eq:delta_min_problem}. Among timestamping data from 47 smartphone models, we observed two classes of timestamping model. On the first kind, finite difference of timestamps follows a Gaussian distribution, as seen in Fig.~\ref{fig:drift}. On the second kind, the smartphone occasionally drops some frames, not shifting the phase but breaking the Gaussian assumption presenting a set of clusters (Fig.~\ref{fig:htc} top-right). Analyzing distribution of every cluster separately, as demonstrated in Fig.~\ref{fig:htc} bottom-right, it could be stated that clusters follow Gaussian distribution. Such decomposition into clusters is done as described in \eqref{eq:delta_min_problem}.

% \gf{I would say here that this allows to break down the problem into sequences that maintain Gaussianity, or soehting lkie that}\gf{updated, ok, so just a reminder, clusters were just described above.}

% Looking for a general method, we break down the time series into small groups of clusters where we can guarantee locally Gaussian conditions, as shown in Fig.~\ref{fig:htc} bottom-right, where indeed these two different clusters present a Gaussian distribution.

% \mf{during the paper it is not shown what rule you use to divide a distribution to Gaussian and non-Gaussian. I see assume phrase after eq (2) for xi, but for the second case there is no clear rule saying is non-gaussian. At least it should be written that we aslo make an assumption: non-Gauss in this case}


% \gf{I think this part could be removed, we simply explain clusters and it is clear... otherwise requires a lot of space just explaning the clustering new formulas, which are the same but with more indexes.}
% Following the idea of clustering from timestamping properties, the problem (\ref{eq:delta_min_problem}) could be decomposed into the sum of minimization problems over clusters $K = \{K_1,..,K_m\}$, where every cluster is defined as $K_i = \{\Delta t_j | \Delta N_j = i\}$:

% \begin{align}
%     \min_{\tau} \sum_{i=1}^{m} \sum_{\Delta t_j \in K_i} (i \tau - \Delta t_j)^2.
% \end{align}

% Assuming, that for every cluster the noise is Gaussian (we observe this on histograms), $\tau_i$ could be calculated for every subproblem as standard solution of LSQ under Markov-Gaussian assumptions:
% \begin{equation}
%     \tau_i = \min_{\tau} \sum_{\Delta t_j \in K_i} (i \tau - \Delta t_j)^2
% \end{equation}

% Finally, estimated period $\tilde{\tau}$ could be calculated as a weighted expectation of $\tau_i$: $\tilde{\tau} = \mathbb{E}_{K}\{\tau_i\}$.


% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.99\columnwidth]{fig/clust_algo.pdf}
%     \caption{\ak{TODO maybe could be dropped}}
%     \label{fig:phase-alg}
% \end{figure}


\subsection{Evaluation of timestamping model} 
For analysis of timestamping model on different Android smartphones, we used Firebase~\cite{firebase} platform that provides application's run and test on physical devices. 47 smartphone models of available smartphones were chosen which cameras satisfy the criteria mentioned in Sec.~\ref{sec:requirements}. For every smartphone, camera timestamps were collected during \SI{1}{\minute} of continuous camera operation~--- \SI{15}{\second} of preview mode, \SI{45}{\second} of video mode ($\approx$ 1800 timestamps per device in total). 

% , where $t = \{t_0,\ldots,t_p\}$~--- is a set of observations, $\tau$, $\tau_0$ are estimated parameters, $N_i$ is calculated as described in (\ref{eq_round}):
% \begin{equation}
%     D(t, \tau_0, \tau) = \frac{1}{p}\sum_{1}^{p}\frac{|\tau_0 + N_i \cdot \tau - t_i|}{t_i - t_0}.
% \end{equation}

To evaluate both phase shift stability after switching from preview mode to video mode and drift of the phase shift over time, we use the drift coefficient metric, which measures drift over time. Phase parameters were estimated using the first 25, 50, 200 observations (``train'' set) from the preview mode. Drift coefficient was estimated on the last 1000 (``test'' set) estimations that contain preview mode, switch to video mode, and video mode, their values are depicted in Fig.~\ref{fig:drift} (right). The majority of models, except early Google Pixel models, have drift coefficient less than \SI{1.2}{\milli\second} per minute on the ``test'' set of timestamps, that allows to make the next conclusions: (1) phase is not shifted during switch from preview to video mode, allowing to use phase alignment for video recording on wide range of smartphones, (2) drift coefficient on majority of smartphones is low enough and could be a worthy analogue to professional systems. Analysis of different ``train'' set size [25; 50; 200] demonstrates that 50 timestamp observations ($\approx$ \SI{2}{\second}) are the optimal condition for phase parameters estimation, lower values lead to the increase of drift coefficient. 

==> IEEE Sensors'21 smartphone sync(2)/src/05_video_sync.tex <==
\section{Experiments}

Evaluation on drift and phase shift stability in the previous section demonstrated that switching camera operating mode from preview to video doesn't shift aligned phases. That means that the libsoftwaresync~\cite{ansari2019wireless} approach on phase shift alignment during preview and then capturing standalone preview photos could be scaled to video recording. The original app was extended with a video recording feature, the automatic algorithm for phase calculation.

\textbf{Light scenes} To evaluate the Android application for synchronized video recording, we used a rig with two Samsung Galaxy S20 smartphones and a light setup described in~\cite{faizullin2021twist}, based on periodical flash blinking and rolling shutter camera property. Five pairs of synchronized videos with a duration of \SI{1}{\minute} were recorded. Then, for every pair of videos, the time difference of capturing light between corresponding synchronized frames was calculated, time difference between corresponding frames among all videos does not exceed \SI{250}{\micro\second}.

\textbf{Panorama stitching} To qualitatively demonstrate synchronization quality, we applied panorama stitching for synchronized stereo video in smartphones on the dynamic scene with a jumping person. CLI interface of Hugin stitching software was used to stitch frame pairs. Stitched video is available via the link \url{https://youtu.be/2AEmuIt5TZc}.


==> IEEE Sensors'21 smartphone sync(2)/src/06_conclusion.tex <==
\section{Conclusion}
This paper answers two tackled research questions. Firstly, phase synchronization could be extended from preview mode to video recording mode without losing synchronization. Secondly, this approach could be scaled to a wide family of Android devices with synchronization drift less than \SI{1.2}{\milli\second} per minute, as we demonstrated on 47 smartphone models. Proposed Android-app was quantitatively and qualitatively verified on the multi-view camera system with Samsung Galaxy S20 smartphones. As a result, we obtained a fully automated publicly-available tool for recording synchronized videos on multiple Android smartphones.



% , demonstrating that the phase shift is not changed after switch from preview to video mode. 

% That means that phase alignment, which is available only during preview mode, is not destroyed when devices start video recording. 

==> IEEE Sensors'21 smartphone sync(2)/trash.tex <==
\subsection{Maintaining the Integrity of the Specifications}

The IEEEtran class file is used to format your paper and style the text. All margins, 
column widths, line spaces, and text fonts are prescribed; please do not 
alter them. You may note peculiarities. For example, the head margin
measures proportionately more than is customary. This measurement 
and others are deliberate, using specifications that anticipate your paper 
as one part of the entire proceedings, and not as an independent document. 
Please do not revise any of the current designations.

\section{Prepare Your Paper Before Styling}
Before you begin to format your paper, first write and save the content as a 
separate text file. Complete all content and organizational editing before 
formatting. Please note sections \ref{AA}--\ref{SCM} below for more information on 
proofreading, spelling and grammar.

Keep your text and graphic files separate until after the text has been 
formatted and styled. Do not number text heads---{\LaTeX} will do that 
for you.

\subsection{Abbreviations and Acronyms}\label{AA}
Define abbreviations and acronyms the first time they are used in the text, 
even after they have been defined in the abstract. Abbreviations such as 
IEEE, SI, MKS, CGS, ac, dc, and rms do not have to be defined. Do not use 
abbreviations in the title or heads unless they are unavoidable.

\subsection{Units}
\begin{itemize}
\item Use either SI (MKS) or CGS as primary units. (SI units are encouraged.) English units may be used as secondary units (in parentheses). An exception would be the use of English units as identifiers in trade, such as ``3.5-inch disk drive''.
\item Avoid combining SI and CGS units, such as current in amperes and magnetic field in oersteds. This often leads to confusion because equations do not balance dimensionally. If you must use mixed units, clearly state the units for each quantity that you use in an equation.
\item Do not mix complete spellings and abbreviations of units: ``Wb/m\textsuperscript{2}'' or ``webers per square meter'', not ``webers/m\textsuperscript{2}''. Spell out units when they appear in text: ``. . . a few henries'', not ``. . . a few H''.
\item Use a zero before decimal points: ``0.25'', not ``.25''. Use ``cm\textsuperscript{3}'', not ``cc''.)
\end{itemize}

\subsection{Equations}
Number equations consecutively. To make your 
equations more compact, you may use the solidus (~/~), the exp function, or 
appropriate exponents. Italicize Roman symbols for quantities and variables, 
but not Greek symbols. Use a long dash rather than a hyphen for a minus 
sign. Punctuate equations with commas or periods when they are part of a 
sentence, as in:
\begin{equation}
a+b=\gamma\label{eq}
\end{equation}

Be sure that the 
symbols in your equation have been defined before or immediately following 
the equation. Use ``\eqref{eq}'', not ``Eq.~\eqref{eq}'' or ``equation \eqref{eq}'', except at 
the beginning of a sentence: ``Equation \eqref{eq} is . . .''

\subsection{\LaTeX-Specific Advice}

Please use ``soft'' (e.g., \verb|\eqref{Eq}|) cross references instead
of ``hard'' references (e.g., \verb|(1)|). That will make it possible
to combine sections, add equations, or change the order of figures or
citations without having to go through the file line by line.

Please don't use the \verb|{eqnarray}| equation environment. Use
\verb|{align}| or \verb|{IEEEeqnarray}| instead. The \verb|{eqnarray}|
environment leaves unsightly spaces around relation symbols.

Please note that the \verb|{subequations}| environment in {\LaTeX}
will increment the main equation counter even when there are no
equation numbers displayed. If you forget that, you might write an
article in which the equation numbers skip from (17) to (20), causing
the copy editors to wonder if you've discovered a new method of
counting.

{\BibTeX} does not work by magic. It doesn't get the bibliographic
data from thin air but from .bib files. If you use {\BibTeX} to produce a
bibliography you must send the .bib files. 

{\LaTeX} can't read your mind. If you assign the same label to a
subsubsection and a table, you might find that Table I has been cross
referenced as Table IV-B3. 

{\LaTeX} does not have precognitive abilities. If you put a
\verb|\label| command before the command that updates the counter it's
supposed to be using, the label will pick up the last counter to be
cross referenced instead. In particular, a \verb|\label| command
should not go before the caption of a figure or a table.

Do not use \verb|\nonumber| inside the \verb|{array}| environment. It
will not stop equation numbers inside \verb|{array}| (there won't be
any anyway) and it might stop a wanted equation number in the
surrounding equation.

\subsection{Some Common Mistakes}\label{SCM}
\begin{itemize}
\item The word ``data'' is plural, not singular.
\item The subscript for the permeability of vacuum $\mu_{0}$, and other common scientific constants, is zero with subscript formatting, not a lowercase letter ``o''.
\item In American English, commas, semicolons, periods, question and exclamation marks are located within quotation marks only when a complete thought or name is cited, such as a title or full quotation. When quotation marks are used, instead of a bold or italic typeface, to highlight a word or phrase, punctuation should appear outside of the quotation marks. A parenthetical phrase or statement at the end of a sentence is punctuated outside of the closing parenthesis (like this). (A parenthetical sentence is punctuated within the parentheses.)
\item A graph within a graph is an ``inset'', not an ``insert''. The word alternatively is preferred to the word ``alternately'' (unless you really mean something that alternates).
\item Do not use the word ``essentially'' to mean ``approximately'' or ``effectively''.
\item In your paper title, if the words ``that uses'' can accurately replace the word ``using'', capitalize the ``u''; if not, keep using lower-cased.
\item Be aware of the different meanings of the homophones ``affect'' and ``effect'', ``complement'' and ``compliment'', ``discreet'' and ``discrete'', ``principal'' and ``principle''.
\item Do not confuse ``imply'' and ``infer''.
\item The prefix ``non'' is not a word; it should be joined to the word it modifies, usually without a hyphen.
\item There is no period after the ``et'' in the Latin abbreviation ``et al.''.
\item The abbreviation ``i.e.'' means ``that is'', and the abbreviation ``e.g.'' means ``for example''.
\end{itemize}
An excellent style manual for science writers is \cite{b7}.

\subsection{Authors and Affiliations}
\textbf{The class file is designed for, but not limited to, six authors.} A 
minimum of one author is required for all conference articles. Author names 
should be listed starting from left to right and then moving down to the 
next line. This is the author sequence that will be used in future citations 
and by indexing services. Names should not be listed in columns nor group by 
affiliation. Please keep your affiliations as succinct as possible (for 
example, do not differentiate among departments of the same organization).

\subsection{Identify the Headings}
Headings, or heads, are organizational devices that guide the reader through 
your paper. There are two types: component heads and text heads.

Component heads identify the different components of your paper and are not 
topically subordinate to each other. Examples include Acknowledgments and 
References and, for these, the correct style to use is ``Heading 5''. Use 
``figure caption'' for your Figure captions, and ``table head'' for your 
table title. Run-in heads, such as ``Abstract'', will require you to apply a 
style (in this case, italic) in addition to the style provided by the drop 
down menu to differentiate the head from the text.

Text heads organize the topics on a relational, hierarchical basis. For 
example, the paper title is the primary text head because all subsequent 
material relates and elaborates on this one topic. If there are two or more 
sub-topics, the next level head (uppercase Roman numerals) should be used 
and, conversely, if there are not at least two sub-topics, then no subheads 
should be introduced.

\subsection{Figures and Tables}
\paragraph{Positioning Figures and Tables} Place figures and tables at the top and 
bottom of columns. Avoid placing them in the middle of columns. Large 
figures and tables may span across both columns. Figure captions should be 
below the figures; table heads should appear above the tables. Insert 
figures and tables after they are cited in the text. Use the abbreviation 
``Fig.~\ref{fig}'', even at the beginning of a sentence.

\begin{table}[htbp]
\caption{Table Type Styles}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Table}&\multicolumn{3}{|c|}{\textbf{Table Column Head}} \\
\cline{2-4} 
\textbf{Head} & \textbf{\textit{Table column subhead}}& \textbf{\textit{Subhead}}& \textbf{\textit{Subhead}} \\
\hline
copy& More table copy$^{\mathrm{a}}$& &  \\
\hline
\multicolumn{4}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
\end{tabular}
\label{tab1}
\end{center}
\end{table}

\begin{figure}[htbp]
\centerline{\includegraphics{fig1.png}}
\caption{Example of a figure caption.}
\label{fig}
\end{figure}

Figure Labels: Use 8 point Times New Roman for Figure labels. Use words 
rather than symbols or abbreviations when writing Figure axis labels to 
avoid confusing the reader. As an example, write the quantity 
``Magnetization'', or ``Magnetization, M'', not just ``M''. If including 
units in the label, present them within parentheses. Do not label axes only 
with units. In the example, write ``Magnetization (A/m)'' or ``Magnetization 
\{A[m(1)]\}'', not just ``A/m''. Do not label axes with a ratio of 
quantities and units. For example, write ``Temperature (K)'', not 
``Temperature/K''.

\section*{Acknowledgment}

The preferred spelling of the word ``acknowledgment'' in America is without 
an ``e'' after the ``g''. Avoid the stilted expression ``one of us (R. B. 
G.) thanks $\ldots$''. Instead, try ``R. B. G. thanks$\ldots$''. Put sponsor 
acknowledgments in the unnumbered footnote on the first page.

\section*{References}

Please number citations consecutively within brackets \cite{b1}. The 
sentence punctuation follows the bracket \cite{b2}. Refer simply to the reference 
number, as in \cite{b3}---do not use ``Ref. \cite{b3}'' or ``reference \cite{b3}'' except at 
the beginning of a sentence: ``Reference \cite{b3} was the first $\ldots$''

\color{red}
All references should be on the 4\textsuperscript{th} page whereas all of the main text should be on the first 3 pages.
\color{black}

Number footnotes separately in superscripts. Place the actual footnote at 
the bottom of the column in which it was cited. Do not put footnotes in the 
abstract or reference list. Use letters for table footnotes.

Unless there are six authors or more give all authors' names; do not use 
``et al.''. Papers that have not been published, even if they have been 
submitted for publication, should be cited as ``unpublished'' \cite{b4}. Papers 
that have been accepted for publication should be cited as ``in press'' \cite{b5}. 
Capitalize only the first word in a paper title, except for proper nouns and 
element symbols.

For papers published in translation journals, please give the English 
citation first, followed by the original foreign-language citation \cite{b6}.

\vspace{12pt}
\color{red}
IEEE conference templates contain guidance text for composing and formatting conference papers. Please ensure that all template text is removed from your conference paper prior to submission to the conference. Failure to remove the template text from your paper may result in your paper not being published.
\color{black}

% Smartphones camera usage: robots, microscopes --- built-in sensors and computational capabilities of smartphones decrease cost of target device where smartphones are employed

% Multi-view, free view-point video


% \begin{align}
%     \min_{\tau_0, \tau, N_1,.., N_s} \sum_{i=1}^{s} (\tau_0 + N_i \cdot \tau - T_i)^2 \\
%     \tau_0, \tau \in \mathbb{R} \\
%     N_i < N_{i + 1}, N_i \in \mathbb{N}
% \end{align}

% \subsection{Mathematical model of timestamping}

% Following those observations, the next timestamping model could be formulated:

% \begin{align}
%     T_i = T_{0} + N_i \cdot \tau + \epsilon \\
%     N_i < N_{i + 1} \\
%     N_i \in \mathbb{N}
% \end{align}

% where $T_i$~--- timestamp of $i$-th frame in smartphone time domain, $T_0$~--- camera module boot time, $N_i$~--- order number of frame if there will not be frame drops, $\tau$~--- frame phase, $\epsilon$~--- noise \ak{Properly define}. $T = \{T_1,.., T_n\}$~--- set of timestamps used for phase estimation.

% Parameters we are interested in are $\tau$ and $T_{0}$. Considering difference between consecutive timestamps the next expression is derived:

% \begin{equation}
%     \Delta T_i = T_{i + 1} - T_i = (N_{i + 1} - N_{i})\cdot \tau + \epsilon_{i + 1} - \epsilon_{i}
% \end{equation}


% % Following notices on frame drops, we consider the next model of frame timestamping

% % \begin{align}
% %     T^m_i = \tau_0 + N_i \cdot \tau \\
% %     N_i \in \mathbb{N}
% % \end{align}

% Given observations of timestamps $T = \{T_1,..,T_s\}$, the task is to get $\tau_0$ and $\tau$ from the next minimization problem:

% \begin{align}
%     \min_{\tau_0, \tau, N_1,.., N_s} \sum_{i=1}^{s} (\tau_0 + N_i \cdot \tau - T_i)^2 \\
%     \tau(N_i - \frac{1}{2}) \leq T_i \leq \tau(N_i + \frac{1}{2}) \\
%     \tau_0, \tau \in \mathbb{R} \\
%     N_i \in \mathbb{N}
% \end{align}

% Only clock synchronization between smartphones using standard network-based (NTP, PTP) or data-based approaches is not enough for video synchronization due to low observation frequency (usually 30 fps). In such a way, the difference between frames capturing could be up to 15msec, which could be crucial for high-dynamic environments. Thus, besides clock synchronization, simultaneous triggering of frame capture from both devices is required.  In smartphones' case, such triggering is complicated because smartphone OS usually provides a high-level API of camera control that doesn't include such an option. To overcome that problem, existing works propose continuously reloading the camera module until the capturing phase will be aligned~\cite{latimer2014socialsync} or requesting frames with different exposure times, which shift phase in a more controllable way~\cite{ansari2019wireless}. Despite the concept of this work is good, it is limited because of the next two reasons: (1) it requires tuning phase for every device manually and (2) it allows only small fps photos making.

% \begin{table}[h]
% \centering
% \label{table:manuf}
% \caption{\ak{RENAME and UPDATE to 47}}
% \begin{tabular}{@{}cc@{}}
% \toprule
% Manufacturer   & Amount      \\ \midrule
% Google         & 5           \\
% LG             & 7           \\
% Samsung        & 20          \\
% Sony           & 4           \\
% Xiaomi         & 3           \\
% Others         & 13          \\ \midrule
% \textbf{Total} & \textbf{52} \\ \bottomrule
% \end{tabular}
% \end{table}

% The scope of Libsoftwaresync is limited to only photos capturing (no video support, which is more useful for robotics and computer vision applications) and to experiments only with Google Pixel smartphones, not giving answers on the applicability of this technology for other smartphone models. An additional obstacle for applying this approach is a not-investigated frame timestamping model that requires manual tuning of frame period parameters for every smartphone. Our research answers all those not-investigated questions for the huge variety of smartphone models.

% \cite{bortolon2021multi} -- multi-view smartphone sync for augmented reality

% \cite{faizullin2021twist} -- twist-n-sync

% \cite{ansari2019wireless} -- google guys sync

% \section{Background}

% \subsection{Google app}
% \outsource{Explanation of Google sync approach}

% \gf{careful here, I would call this NTP-based min time sync. not google, that is informal name we use.}
% Principle of work -- two-step algorithm that first sync time domains and then shift phase of frames

% Lacks?

% \subsection{Periodicity?}

% \ak{Not sure, think}


% \begin{table}[]
% \centering
% \caption{\ak{TODO}}
% \begin{tabular}{ccc}
% \# & \begin{tabular}[c]{@{}c@{}}Frame pairs amount\end{tabular} & \begin{tabular}[c]{@{}l@{}}Synchronization error ($\muup$sec)\end{tabular} \\
% 1 & 1098 & \AK{Present stat} \\
% 2 & 1183 & 0 \\
% 3 & 1167 & 0 \\
% 4 & 1156 & 0 \\
% 5 & 1054 & 0
% \end{tabular}
% \label{table:light}
% \end{table}

% {\footnotesize \textsuperscript{*}Note: Sub-titles are not captured in Xplore and
% should not be used}
% \thanks{Identify applicable funding agency here. If none, delete this.}

% \author{\IEEEauthorblockN{Azat Akhmetyanov}
% \IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
% \textit{name of organization (of Aff.)}\\
% City, Country \\
% email address or ORCID}
% \and
% \IEEEauthorblockN{Anastasiia Kornilova}
% \IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
% \textit{name of organization (of Aff.)}\\
% City, Country \\
% email address or ORCID}
% \and
% \IEEEauthorblockN{Marsel Faizullin}
% \IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
% \textit{name of organization (of Aff.)}\\
% City, Country \\
% email address or ORCID}
% \and
% \IEEEauthorblockN{Gonzalo Ferrer}
% \IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
% \textit{name of organization (of Aff.)}\\
% City, Country \\
% email address or ORCID}
% }

% GF: not sure if this now is of any help, maybe better later.
%Usually, the user requires to tune the parameters manually for every smartphone. Knowing these parameters, a target phase \gf{shift?} $\tau_i^0$ could be chosen for all nodes in the system after an optimization process that estimates the timestamps from this target model. Generalization of this model for the Android family and algorithm for parameters calculation is necessary to analyze phase stability during the switch between preview and video modes and automate the synchronization process.

% Assumption: subsequences of timestamps follow a Gaussian distribution, and we require clusterization to find the change point to apply the LSQ.  

% \begin{align}
%     \min_{\tau_0,\tau} \quad \sum_{i=1}^{s} \left(\tau_0 + N_i(\tau, \tau_0) \cdot \tau - t_i\right)^2 \\ 
%     N_i(\tau, \tau_0) =  \floor*{\frac{t_i - \tau_0}{\tau} + 0.5} \\
%     0 \leq \tau_0 < \tau 
% \end{align}

% \begin{align}
%     \Delta t_i = t_{i + 1} - t_i, \quad
%     \tau_{init} = \min_{i \in [1, s-1]} \Delta t_i \\
%     N_i = \floor*{\frac{t_i}{\tau_{init}}}
% \end{align}


%In order to develop a timestamping model, we take the next two observations of the difference between consecutive timestamps as a basis for timestamping model. The first timestamping behavior is depicted in Fig.~\ref{fig:phase-noise} and demonstrates approximately symmetric deviation of timestamps difference along timestamping period. Fig.~\ref{fig:phase-drops} presents cases when the timestamp difference is a multiple of timestamping periods. That behavior could be interpreted that the camera module drops some frames, but timestamping phase remains the same that doesn't affect synchronization.

% \begin{figure}[h]
%     \centering
%     %\includegraphics[width=0.99\columnwidth]{fig/phase_noise.pdf}
%     \caption{Demonstration of timestamping noise}
%     \label{fig:phase-noise}
% \end{figure}

% \begin{figure}[h]
%     \centering
%     %\includegraphics[width=0.99\columnwidth]{fig/phase_drops.pdf}
%     \caption{Demonstration of frame drops that don't affect phase}
%     \label{fig:phase-drops}
% \end{figure}

% \ak{reformulated}

% Original problem formulation:

% \begin{align}
%     t_1 = \tau_0 + N_1 \tau \\
%     \ldots \\ 
%     t_s = \tau_0 + N_s \tau
% \end{align}

% Equivalent without $\tau_0$:

% \begin{align}
%     t_2 - t_1 = (N_2 - N_1) \tau + \eta_2  - \eta_1 \\
%     \ldots \\ 
%     t_s - t_{s-1} = (N_s - N_{s-1}) \tau
% \end{align}

% \begin{align}
%     \min (\Delta t_i - N \tau)
% \end{align}

==> trash.tex <==
\subsection{Maintaining the Integrity of the Specifications}

The IEEEtran class file is used to format your paper and style the text. All margins, 
column widths, line spaces, and text fonts are prescribed; please do not 
alter them. You may note peculiarities. For example, the head margin
measures proportionately more than is customary. This measurement 
and others are deliberate, using specifications that anticipate your paper 
as one part of the entire proceedings, and not as an independent document. 
Please do not revise any of the current designations.

\section{Prepare Your Paper Before Styling}
Before you begin to format your paper, first write and save the content as a 
separate text file. Complete all content and organizational editing before 
formatting. Please note sections \ref{AA}--\ref{SCM} below for more information on 
proofreading, spelling and grammar.

Keep your text and graphic files separate until after the text has been 
formatted and styled. Do not number text heads---{\LaTeX} will do that 
for you.

\subsection{Abbreviations and Acronyms}\label{AA}
Define abbreviations and acronyms the first time they are used in the text, 
even after they have been defined in the abstract. Abbreviations such as 
IEEE, SI, MKS, CGS, ac, dc, and rms do not have to be defined. Do not use 
abbreviations in the title or heads unless they are unavoidable.

\subsection{Units}
\begin{itemize}
\item Use either SI (MKS) or CGS as primary units. (SI units are encouraged.) English units may be used as secondary units (in parentheses). An exception would be the use of English units as identifiers in trade, such as ``3.5-inch disk drive''.
\item Avoid combining SI and CGS units, such as current in amperes and magnetic field in oersteds. This often leads to confusion because equations do not balance dimensionally. If you must use mixed units, clearly state the units for each quantity that you use in an equation.
\item Do not mix complete spellings and abbreviations of units: ``Wb/m\textsuperscript{2}'' or ``webers per square meter'', not ``webers/m\textsuperscript{2}''. Spell out units when they appear in text: ``. . . a few henries'', not ``. . . a few H''.
\item Use a zero before decimal points: ``0.25'', not ``.25''. Use ``cm\textsuperscript{3}'', not ``cc''.)
\end{itemize}

\subsection{Equations}
Number equations consecutively. To make your 
equations more compact, you may use the solidus (~/~), the exp function, or 
appropriate exponents. Italicize Roman symbols for quantities and variables, 
but not Greek symbols. Use a long dash rather than a hyphen for a minus 
sign. Punctuate equations with commas or periods when they are part of a 
sentence, as in:
\begin{equation}
a+b=\gamma\label{eq}
\end{equation}

Be sure that the 
symbols in your equation have been defined before or immediately following 
the equation. Use ``\eqref{eq}'', not ``Eq.~\eqref{eq}'' or ``equation \eqref{eq}'', except at 
the beginning of a sentence: ``Equation \eqref{eq} is . . .''

\subsection{\LaTeX-Specific Advice}

Please use ``soft'' (e.g., \verb|\eqref{Eq}|) cross references instead
of ``hard'' references (e.g., \verb|(1)|). That will make it possible
to combine sections, add equations, or change the order of figures or
citations without having to go through the file line by line.

Please don't use the \verb|{eqnarray}| equation environment. Use
\verb|{align}| or \verb|{IEEEeqnarray}| instead. The \verb|{eqnarray}|
environment leaves unsightly spaces around relation symbols.

Please note that the \verb|{subequations}| environment in {\LaTeX}
will increment the main equation counter even when there are no
equation numbers displayed. If you forget that, you might write an
article in which the equation numbers skip from (17) to (20), causing
the copy editors to wonder if you've discovered a new method of
counting.

{\BibTeX} does not work by magic. It doesn't get the bibliographic
data from thin air but from .bib files. If you use {\BibTeX} to produce a
bibliography you must send the .bib files. 

{\LaTeX} can't read your mind. If you assign the same label to a
subsubsection and a table, you might find that Table I has been cross
referenced as Table IV-B3. 

{\LaTeX} does not have precognitive abilities. If you put a
\verb|\label| command before the command that updates the counter it's
supposed to be using, the label will pick up the last counter to be
cross referenced instead. In particular, a \verb|\label| command
should not go before the caption of a figure or a table.

Do not use \verb|\nonumber| inside the \verb|{array}| environment. It
will not stop equation numbers inside \verb|{array}| (there won't be
any anyway) and it might stop a wanted equation number in the
surrounding equation.

\subsection{Some Common Mistakes}\label{SCM}
\begin{itemize}
\item The word ``data'' is plural, not singular.
\item The subscript for the permeability of vacuum $\mu_{0}$, and other common scientific constants, is zero with subscript formatting, not a lowercase letter ``o''.
\item In American English, commas, semicolons, periods, question and exclamation marks are located within quotation marks only when a complete thought or name is cited, such as a title or full quotation. When quotation marks are used, instead of a bold or italic typeface, to highlight a word or phrase, punctuation should appear outside of the quotation marks. A parenthetical phrase or statement at the end of a sentence is punctuated outside of the closing parenthesis (like this). (A parenthetical sentence is punctuated within the parentheses.)
\item A graph within a graph is an ``inset'', not an ``insert''. The word alternatively is preferred to the word ``alternately'' (unless you really mean something that alternates).
\item Do not use the word ``essentially'' to mean ``approximately'' or ``effectively''.
\item In your paper title, if the words ``that uses'' can accurately replace the word ``using'', capitalize the ``u''; if not, keep using lower-cased.
\item Be aware of the different meanings of the homophones ``affect'' and ``effect'', ``complement'' and ``compliment'', ``discreet'' and ``discrete'', ``principal'' and ``principle''.
\item Do not confuse ``imply'' and ``infer''.
\item The prefix ``non'' is not a word; it should be joined to the word it modifies, usually without a hyphen.
\item There is no period after the ``et'' in the Latin abbreviation ``et al.''.
\item The abbreviation ``i.e.'' means ``that is'', and the abbreviation ``e.g.'' means ``for example''.
\end{itemize}
An excellent style manual for science writers is \cite{b7}.

\subsection{Authors and Affiliations}
\textbf{The class file is designed for, but not limited to, six authors.} A 
minimum of one author is required for all conference articles. Author names 
should be listed starting from left to right and then moving down to the 
next line. This is the author sequence that will be used in future citations 
and by indexing services. Names should not be listed in columns nor group by 
affiliation. Please keep your affiliations as succinct as possible (for 
example, do not differentiate among departments of the same organization).

\subsection{Identify the Headings}
Headings, or heads, are organizational devices that guide the reader through 
your paper. There are two types: component heads and text heads.

Component heads identify the different components of your paper and are not 
topically subordinate to each other. Examples include Acknowledgments and 
References and, for these, the correct style to use is ``Heading 5''. Use 
``figure caption'' for your Figure captions, and ``table head'' for your 
table title. Run-in heads, such as ``Abstract'', will require you to apply a 
style (in this case, italic) in addition to the style provided by the drop 
down menu to differentiate the head from the text.

Text heads organize the topics on a relational, hierarchical basis. For 
example, the paper title is the primary text head because all subsequent 
material relates and elaborates on this one topic. If there are two or more 
sub-topics, the next level head (uppercase Roman numerals) should be used 
and, conversely, if there are not at least two sub-topics, then no subheads 
should be introduced.

\subsection{Figures and Tables}
\paragraph{Positioning Figures and Tables} Place figures and tables at the top and 
bottom of columns. Avoid placing them in the middle of columns. Large 
figures and tables may span across both columns. Figure captions should be 
below the figures; table heads should appear above the tables. Insert 
figures and tables after they are cited in the text. Use the abbreviation 
``Fig.~\ref{fig}'', even at the beginning of a sentence.

\begin{table}[htbp]
\caption{Table Type Styles}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Table}&\multicolumn{3}{|c|}{\textbf{Table Column Head}} \\
\cline{2-4} 
\textbf{Head} & \textbf{\textit{Table column subhead}}& \textbf{\textit{Subhead}}& \textbf{\textit{Subhead}} \\
\hline
copy& More table copy$^{\mathrm{a}}$& &  \\
\hline
\multicolumn{4}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
\end{tabular}
\label{tab1}
\end{center}
\end{table}

\begin{figure}[htbp]
\centerline{\includegraphics{fig1.png}}
\caption{Example of a figure caption.}
\label{fig}
\end{figure}

Figure Labels: Use 8 point Times New Roman for Figure labels. Use words 
rather than symbols or abbreviations when writing Figure axis labels to 
avoid confusing the reader. As an example, write the quantity 
``Magnetization'', or ``Magnetization, M'', not just ``M''. If including 
units in the label, present them within parentheses. Do not label axes only 
with units. In the example, write ``Magnetization (A/m)'' or ``Magnetization 
\{A[m(1)]\}'', not just ``A/m''. Do not label axes with a ratio of 
quantities and units. For example, write ``Temperature (K)'', not 
``Temperature/K''.

\section*{Acknowledgment}

The preferred spelling of the word ``acknowledgment'' in America is without 
an ``e'' after the ``g''. Avoid the stilted expression ``one of us (R. B. 
G.) thanks $\ldots$''. Instead, try ``R. B. G. thanks$\ldots$''. Put sponsor 
acknowledgments in the unnumbered footnote on the first page.

\section*{References}

Please number citations consecutively within brackets \cite{b1}. The 
sentence punctuation follows the bracket \cite{b2}. Refer simply to the reference 
number, as in \cite{b3}---do not use ``Ref. \cite{b3}'' or ``reference \cite{b3}'' except at 
the beginning of a sentence: ``Reference \cite{b3} was the first $\ldots$''

\color{red}
All references should be on the 4\textsuperscript{th} page whereas all of the main text should be on the first 3 pages.
\color{black}

Number footnotes separately in superscripts. Place the actual footnote at 
the bottom of the column in which it was cited. Do not put footnotes in the 
abstract or reference list. Use letters for table footnotes.

Unless there are six authors or more give all authors' names; do not use 
``et al.''. Papers that have not been published, even if they have been 
submitted for publication, should be cited as ``unpublished'' \cite{b4}. Papers 
that have been accepted for publication should be cited as ``in press'' \cite{b5}. 
Capitalize only the first word in a paper title, except for proper nouns and 
element symbols.

For papers published in translation journals, please give the English 
citation first, followed by the original foreign-language citation \cite{b6}.

\vspace{12pt}
\color{red}
IEEE conference templates contain guidance text for composing and formatting conference papers. Please ensure that all template text is removed from your conference paper prior to submission to the conference. Failure to remove the template text from your paper may result in your paper not being published.
\color{black}

% Smartphones camera usage: robots, microscopes --- built-in sensors and computational capabilities of smartphones decrease cost of target device where smartphones are employed

% Multi-view, free view-point video


% \begin{align}
%     \min_{\tau_0, \tau, N_1,.., N_s} \sum_{i=1}^{s} (\tau_0 + N_i \cdot \tau - T_i)^2 \\
%     \tau_0, \tau \in \mathbb{R} \\
%     N_i < N_{i + 1}, N_i \in \mathbb{N}
% \end{align}

% \subsection{Mathematical model of timestamping}

% Following those observations, the next timestamping model could be formulated:

% \begin{align}
%     T_i = T_{0} + N_i \cdot \tau + \epsilon \\
%     N_i < N_{i + 1} \\
%     N_i \in \mathbb{N}
% \end{align}

% where $T_i$~--- timestamp of $i$-th frame in smartphone time domain, $T_0$~--- camera module boot time, $N_i$~--- order number of frame if there will not be frame drops, $\tau$~--- frame phase, $\epsilon$~--- noise \ak{Properly define}. $T = \{T_1,.., T_n\}$~--- set of timestamps used for phase estimation.

% Parameters we are interested in are $\tau$ and $T_{0}$. Considering difference between consecutive timestamps the next expression is derived:

% \begin{equation}
%     \Delta T_i = T_{i + 1} - T_i = (N_{i + 1} - N_{i})\cdot \tau + \epsilon_{i + 1} - \epsilon_{i}
% \end{equation}


% % Following notices on frame drops, we consider the next model of frame timestamping

% % \begin{align}
% %     T^m_i = \tau_0 + N_i \cdot \tau \\
% %     N_i \in \mathbb{N}
% % \end{align}

% Given observations of timestamps $T = \{T_1,..,T_s\}$, the task is to get $\tau_0$ and $\tau$ from the next minimization problem:

% \begin{align}
%     \min_{\tau_0, \tau, N_1,.., N_s} \sum_{i=1}^{s} (\tau_0 + N_i \cdot \tau - T_i)^2 \\
%     \tau(N_i - \frac{1}{2}) \leq T_i \leq \tau(N_i + \frac{1}{2}) \\
%     \tau_0, \tau \in \mathbb{R} \\
%     N_i \in \mathbb{N}
% \end{align}

% Only clock synchronization between smartphones using standard network-based (NTP, PTP) or data-based approaches is not enough for video synchronization due to low observation frequency (usually 30 fps). In such a way, the difference between frames capturing could be up to 15msec, which could be crucial for high-dynamic environments. Thus, besides clock synchronization, simultaneous triggering of frame capture from both devices is required.  In smartphones' case, such triggering is complicated because smartphone OS usually provides a high-level API of camera control that doesn't include such an option. To overcome that problem, existing works propose continuously reloading the camera module until the capturing phase will be aligned~\cite{latimer2014socialsync} or requesting frames with different exposure times, which shift phase in a more controllable way~\cite{ansari2019wireless}. Despite the concept of this work is good, it is limited because of the next two reasons: (1) it requires tuning phase for every device manually and (2) it allows only small fps photos making.

% \begin{table}[h]
% \centering
% \label{table:manuf}
% \caption{\ak{RENAME and UPDATE to 47}}
% \begin{tabular}{@{}cc@{}}
% \toprule
% Manufacturer   & Amount      \\ \midrule
% Google         & 5           \\
% LG             & 7           \\
% Samsung        & 20          \\
% Sony           & 4           \\
% Xiaomi         & 3           \\
% Others         & 13          \\ \midrule
% \textbf{Total} & \textbf{52} \\ \bottomrule
% \end{tabular}
% \end{table}

% The scope of Libsoftwaresync is limited to only photos capturing (no video support, which is more useful for robotics and computer vision applications) and to experiments only with Google Pixel smartphones, not giving answers on the applicability of this technology for other smartphone models. An additional obstacle for applying this approach is a not-investigated frame timestamping model that requires manual tuning of frame period parameters for every smartphone. Our research answers all those not-investigated questions for the huge variety of smartphone models.

% \cite{bortolon2021multi} -- multi-view smartphone sync for augmented reality

% \cite{faizullin2021twist} -- twist-n-sync

% \cite{ansari2019wireless} -- google guys sync

% \section{Background}

% \subsection{Google app}
% \outsource{Explanation of Google sync approach}

% \gf{careful here, I would call this NTP-based min time sync. not google, that is informal name we use.}
% Principle of work -- two-step algorithm that first sync time domains and then shift phase of frames

% Lacks?

% \subsection{Periodicity?}

% \ak{Not sure, think}


% \begin{table}[]
% \centering
% \caption{\ak{TODO}}
% \begin{tabular}{ccc}
% \# & \begin{tabular}[c]{@{}c@{}}Frame pairs amount\end{tabular} & \begin{tabular}[c]{@{}l@{}}Synchronization error ($\muup$sec)\end{tabular} \\
% 1 & 1098 & \AK{Present stat} \\
% 2 & 1183 & 0 \\
% 3 & 1167 & 0 \\
% 4 & 1156 & 0 \\
% 5 & 1054 & 0
% \end{tabular}
% \label{table:light}
% \end{table}

% {\footnotesize \textsuperscript{*}Note: Sub-titles are not captured in Xplore and
% should not be used}
% \thanks{Identify applicable funding agency here. If none, delete this.}

% \author{\IEEEauthorblockN{Azat Akhmetyanov}
% \IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
% \textit{name of organization (of Aff.)}\\
% City, Country \\
% email address or ORCID}
% \and
% \IEEEauthorblockN{Anastasiia Kornilova}
% \IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
% \textit{name of organization (of Aff.)}\\
% City, Country \\
% email address or ORCID}
% \and
% \IEEEauthorblockN{Marsel Faizullin}
% \IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
% \textit{name of organization (of Aff.)}\\
% City, Country \\
% email address or ORCID}
% \and
% \IEEEauthorblockN{Gonzalo Ferrer}
% \IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
% \textit{name of organization (of Aff.)}\\
% City, Country \\
% email address or ORCID}
% }

% GF: not sure if this now is of any help, maybe better later.
%Usually, the user requires to tune the parameters manually for every smartphone. Knowing these parameters, a target phase \gf{shift?} $\tau_i^0$ could be chosen for all nodes in the system after an optimization process that estimates the timestamps from this target model. Generalization of this model for the Android family and algorithm for parameters calculation is necessary to analyze phase stability during the switch between preview and video modes and automate the synchronization process.

% Assumption: subsequences of timestamps follow a Gaussian distribution, and we require clusterization to find the change point to apply the LSQ.  

% \begin{align}
%     \min_{\tau_0,\tau} \quad \sum_{i=1}^{s} \left(\tau_0 + N_i(\tau, \tau_0) \cdot \tau - t_i\right)^2 \\ 
%     N_i(\tau, \tau_0) =  \floor*{\frac{t_i - \tau_0}{\tau} + 0.5} \\
%     0 \leq \tau_0 < \tau 
% \end{align}

% \begin{align}
%     \Delta t_i = t_{i + 1} - t_i, \quad
%     \tau_{init} = \min_{i \in [1, s-1]} \Delta t_i \\
%     N_i = \floor*{\frac{t_i}{\tau_{init}}}
% \end{align}


%In order to develop a timestamping model, we take the next two observations of the difference between consecutive timestamps as a basis for timestamping model. The first timestamping behavior is depicted in Fig.~\ref{fig:phase-noise} and demonstrates approximately symmetric deviation of timestamps difference along timestamping period. Fig.~\ref{fig:phase-drops} presents cases when the timestamp difference is a multiple of timestamping periods. That behavior could be interpreted that the camera module drops some frames, but timestamping phase remains the same that doesn't affect synchronization.

% \begin{figure}[h]
%     \centering
%     %\includegraphics[width=0.99\columnwidth]{fig/phase_noise.pdf}
%     \caption{Demonstration of timestamping noise}
%     \label{fig:phase-noise}
% \end{figure}

% \begin{figure}[h]
%     \centering
%     %\includegraphics[width=0.99\columnwidth]{fig/phase_drops.pdf}
%     \caption{Demonstration of frame drops that don't affect phase}
%     \label{fig:phase-drops}
% \end{figure}

% \ak{reformulated}

% Original problem formulation:

% \begin{align}
%     t_1 = \tau_0 + N_1 \tau \\
%     \ldots \\ 
%     t_s = \tau_0 + N_s \tau
% \end{align}

% Equivalent without $\tau_0$:

% \begin{align}
%     t_2 - t_1 = (N_2 - N_1) \tau + \eta_2  - \eta_1 \\
%     \ldots \\ 
%     t_s - t_{s-1} = (N_s - N_{s-1}) \tau
% \end{align}

% \begin{align}
%     \min (\Delta t_i - N \tau)
% \end{align}
